Computing second-order points under equality constraints: revisiting Fletcher's augmented Lagrangian

We address the problem of minimizing a smooth function under smooth equality constraints. Under regularity assumptions on these constraints, we propose a notion of approximate first- and second-order critical point which relies on the geometric formalism of Riemannian optimization. Using a smooth exact penalty function known as Fletcher's augmented Lagrangian, we propose an algorithm to minimize the penalized cost function which reaches $\varepsilon$-approximate second-order critical points of the original optimization problem in at most $\mathcal{O}(\varepsilon^{-3})$ iterations. This improves on current best theoretical bounds. Along the way, we show new properties of Fletcher's augmented Lagrangian, which may be of independent interest.

==> preamble_fletcher.tex <==

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
%\usepackage{lmodern}
%\usepackage{circuitikz}
\usepackage{color}
\usepackage{wrapfig}
\usepackage{placeins}
%\usepackage{slashbox}
\usepackage{subfigure}
\usepackage{tabu}
\usepackage{fullpage}
\usepackage[squaren]{SIunits}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage[pdftex]{graphicx}
\usepackage{epstopdf}
\usepackage{epsfig}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\usepackage[colorlinks=true,bookmarks=false,linkcolor=blue,urlcolor=blue,citecolor=blue,breaklinks=true]{hyperref}
\usepackage{breakcites}
\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{eurosym}
\usepackage{amsmath}
\numberwithin{equation}{section}
\usepackage{amssymb}
%\usepackage{ulem}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{blkarray}
\usepackage{dsfont}% use $\mathds{1}$
\usepackage{comment}
\usepackage{rotating}
\newcommand{\C}{\mathrm{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\red}{\textcolor{red}}
\definecolor{purple}{rgb}{0.74, 0.2, 0.64}
\newcommand{\purple}{\textcolor{purple}}

\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\ddt}{\frac{\mathrm{d}}{\mathrm{d}t}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\Lcalb}{\mathcal{L}_\beta}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\change}{\textcolor{blue}}
\newcommand{\flo}{\textcolor{red}}
\newcommand{\dis}{\displaystyle}
\newcommand{\dr}{\partial}
\newcommand{\txt}{\text}
\newcommand{\transpose}{^\top}
\newcommand{\td}{\todo[inline]}
\newcommand{\ttt}{\texttt}
\newcommand{\itt}{\textit}
\newcommand{\mcal}{\mathcal}
\newcommand{\St}{\mathrm{St}}
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\col}{\mathrm{col}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\Hess}{\mathrm{Hess}}
\newcommand{\hess}{\nabla^2}
\newcommand{\LAb}{\mathrm{L}_{\Acal,b}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\Prm}{\mathrm{P}}
\newcommand{\Sym}{\mathrm{Sym}}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\spann}{\operatorname{span}}
\newcommand{\nl}{\newline}
\newcommand{\inner}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\I}{\mathrm{I}}
\newcommand{\sigmamin}{\sigma_\mathrm{min}}
\newcommand{\sigmamax}{\sigma_\mathrm{max}}
\newcommand{\sigmabar}{\underline{\sigma}}
\newcommand{\Clambdabar}{\overline{C_{\lambda}}}
\newcommand{\betabar}{\overline{\beta}}
\newcommand{\lambdamin}{\lambda_\mathrm{min}}
\newcommand{\LP}{\mathrm{LP}}
\newcommand{\tmax}{t_{\mathrm{max}}}

\usepackage{bm}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Gr}{\mathrm{Grass}}
\newcommand{\Null}{\mathrm{null}}
\newcommand{\Retr}{\mathrm{Retr}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\Grass}{\mathrm{Grass}}
\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{algorithmicx}%
\usepackage{algpseudocode}
\usepackage{todonotes}
\def \SVD {\mathrm{SVD}}

%\DeclareMathOperator{\cosh}{cosh}%
%\DeclareMathOperator{\acosh}{acosh}
%\DeclareMathOperator{\arcos}{arcos}

\newcommand{\aref}[1]{\hyperref[#1]{A\ref{#1}}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_\mathrm{F}}
\newcommand{\opnorm}[1]{\left\|{#1}\right\|_\mathrm{op}}
%\newcommand{\frobnorm}[2][F]{\left\|{#2}\right\|_\mathrm{#1}}
%\newcommand{\fronormbig}[1]{\big\|{#1}\big\|_\mathrm{F}}

\usepackage{apxproof}
\newtheorem{theorem}			     {Theorem}	[section]
%\newtheorem{proposition}[theorem]	 {Proposition}	
%\newtheoremrep{theorem}			     {Theorem}	[section]
\newtheorem{corollary}	  [theorem]	 {Corollary}	
\newtheorem{lemma}	      [theorem]  {Lemma}		
\newtheorem{definition}	         {Definition}[section]
\newtheorem{assumption} {A\ignorespaces}%[section]
%\theoremstyle{definition}
\newtheorem{remark}{Remark}[section]
\newtheorem*{example*}{Example}
\newtheoremrep{proposition} [theorem] {Proposition}
\newtheorem{claim}			     {Claim}	[section]
\newtheorem{testcase}			     {Case study}	[section]
%\newtheorem{contreexemple}[exemple]{Contre-exemple}
%\newtheorem{probleme}	             {Probl\`eme}[chapter]
%\newtheoremrep{examplerep}{Example}[section]

\usepackage{listings}
\usepackage{textcomp}
\definecolor{listinggray}{gray}{0.9}
\definecolor{lbcolor}{rgb}{0.9,0.9,0.9}
\lstset{
	backgroundcolor=\color{lbcolor},
	tabsize=4,
	rulecolor=,
	language=matlab,
        basicstyle=\scriptsize,
        upquote=true,
        aboveskip={1.5\baselineskip},
        columns=fixed,
        showstringspaces=false,
        extendedchars=true,
        breaklines=true,
        prebreak = \raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
        frame=single,
        showtabs=false,
        showspaces=false,
        showstringspaces=false,
        identifierstyle=\ttfamily,
        keywordstyle=\color[rgb]{0,0,1},
        commentstyle=\color[rgb]{0.133,0.545,0.133},
        stringstyle=\color[rgb]{0.627,0.126,0.941},
}

\DeclareMathOperator{\e}{e}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs=false}


\newcommand{\vone}{\textcolor{blue}}

